PlanIt: A Crowdsourcing Approach for Learning to Plan Paths from Large Scale Preference Feedback

We consider the problem of learning user preferences over robot trajectories for environments rich in objects and humans. This is challenging because the criterion defining a good trajectory varies with users, tasks and interactions in the environment. We represent trajectory preferences using a cost function that the robot learns and uses it to generate good trajectories in new environments. We design a crowdsourcing system - PlanIt, where non-expert users label segments of the robot's trajectory. PlanIt allows us to collect a large amount of user feedback, and using the weak and noisy labels from PlanIt we learn the parameters of our model. We test our approach on 122 different environments for robotic navigation and manipulation tasks. Our extensive experiments show that the learned cost function generates preferred trajectories in human environments. Our crowdsourcing system is publicly available for the visualization of the learned costs and for providing preference feedback: \url{http://planit.cs.cornell.edu}

==> humanfeedback.tex <==
\section{\textit{Planit} Engine}


==> planit.tex <==
% !TEX root = writeup.tex

\section{PlanIt: An Engine for Online Preference Rating for Trajectories}
\label{subsec:planit}
\begin{figure*}[t]
\centering
\includegraphics[width=.7\linewidth]{planit4.png}
\caption{\textbf{Our PlanIt Interface}: In this example, a video is shown of an environment 
with two humans. One human is walking towards the door while the other is browsing books. 
The context is displayed for the human labeler to read. On the navigation time-bar below, 
the time interval where the robot crosses the human browsing books is colored in red by the 
user, and the interval when the robot carefully avoids the walking human is colored in green.}
\label{fig:planit}
\end{figure*}



We train our model with data collected from non-expert users.  In the past, rich data along with principled learning algorithms 
have achieved success in many robotic applications. For example, Curtis et al.~\cite{Curtis08} learned to grasp novel
objects using the GraspIt!~\cite{Miller04} database. Paolini et al.~\cite{Paolini13} 
modeled post-grasp manipulation over thousands of grasp trails. Data-driven
approaches have assisted manipulation tasks in unstructured environments~\cite{Katz08} and
modeling of high-dimensional trajectories~\cite{Vernaza12}.
Inspired by these previous works, we take a data-driven approach to
learning preferences and to this end, we design \emph{PlanIt}: a scalable approach 
for collecting preference data over trajectories:
\\~
\hspace*{.5cm}\url{http://planit.cs.cornell.edu}
\\
\begin{figure}[t]
\centering
\begin{tabular}{@{\hskip -.1in}c@{\hskip -.2in}c@{\hskip -.1in}}
\subfigure[Watching]{
\includegraphics[width=.5\linewidth,height=.33\linewidth]{betaplot_task_bedroom_activity_watching.png}
}
&
\subfigure[Interacting]{
\includegraphics[width=.5\linewidth,height=.33\linewidth]{betaplot_task_bedroom_activity_interacting.png}
}
\end{tabular}
\caption{\textbf{Result of learned edge preference.} Distance between human and
object is normalized to 1. Human is at 0 and object at 1. For interacting
activity, edge preference is symmetric between two humans, but for watching
activity humans do not prefer the robot passing right from front.}
\label{fig:edge-pref}
\end{figure}

In learning-based approaches in previous works, 
users can reveal their preferences over trajectories in multiple ways:
\begin{enumerate}
\item \emph{Learning from Demonstration:} An expert demonstrates optimal
trajectory on the robot. This approach has accomplished many challenging
robotic tasks~\cite{Abbeel10,Kober11,Ratliff06}. However it requires an expert
to provide the demonstrations. We are interested in learning preferences of
users and not that of an expert. Further, it is applicable to  
scenarios when it is clear to an expert what constitutes a good trajectory.
\item \emph{Keyframe-based Demonstration:}  it is similar to LfD but instead of
demonstrating the complete trajectory, an expert demonstrates only the relevant 
keyframes~\cite{Akgun12}.
\item \emph{Co-active Learning, Iteratively providing incremental feedback:} In
this approach, a non-expert user iteratively improves the trajectory proposed by
the robot~\cite{Jain13,Jain13b}. Through multiple feedback iterations, the user
guides the robot to the correct trajectory instead of providing the optimal
demonstrations. 
\end{enumerate}
The above mentioned approaches are limited by the amount of user
preference data they can elicit. In both LfD and co-active learning, it is time consuming and
expensive to collect preference data over many environments with the robot system. 
However, one of our main objective is to learn with preference data from \textit{non-expert} 
users over a large number of  environments. Further, previous approaches elicit
demonstrations for specific robotic tasks, while we are interested in learning
generic affordance representations that could be used in new situations.   

\smallskip
\noindent
\emph{User feedback method in PlanIt:}
Our goal is to obtain large-scale data of user preferences in a wide-variety of
environments. To this end, we develop an application where users watch videos of the robot
navigating in context-rich environments and indicate their preferences, i.e.,
likes or dislikes, by labeling segments of the video (Fig.~\ref{fig:planit}). 
In particular, we keep it simple for users by providing three choices
\{\textit{bad, neutral, good}\}, using which users label time intervals of the video.
For example, trajectory segments where the robot passes between a human and a TV 
can be labeled as bad, and segments where the robot navigates in open space as
neutral.

If the user is presented with trajectory $\mathcal{T}$ then one
possible user preference can be  three sub-trajectories
$\mathcal{T}^{(1)}_g,\mathcal{T}^{(2)}_b,\mathcal{T}^{(3)}_n \in \mathcal{T}$ labeled as
good, bad and neutral respectively. For the ease of usability and to reduce
labeling effort, users only provide the label and do not reveal the
(\textit{latent}) reason for their label or the activity which the trajectory
interacts with (an environment can have multiple activities,
Fig.~\ref{fig:activities}, \ref{fig:generative} left). 
%As an example a user could label a trajectory segment as bad because it interferes with multiple activities.
We capture the user's intention as a latent variable 
during learning (Section~\ref{subsec:learning}). %In Section~\ref{sec:experiment} we give 
%details of the user preference data we collect from PlanIt and ways to generate
%robot navigation videos.

\smallskip
\noindent
\textit{Generating robot navigation trajectory and videos:} We use OpenRAVE~\cite{Diankov10}
and sample many trajectories (using RRT~\cite{Lavalle01}) of PR2 navigating in
human environments. We video record these trajectories and add them to PlanIt database. Currently, our
database has 2500 trajectories over 122 environments (described in
Section~\ref{sec:experiment},), and is continuously growing in size. 
Users watch PR2
interact with human activities through these videos and reveal their preferences. % Of note, 
We also ensure that the trajectories in database are diverse, following ideas
presented in \cite{Berg10,Jain13}.
%in the environment. Based of these interactions users reveal their preferences.


==> system.tex <==
% !TEX root = writeup.tex
\section{System Overview}
\label{sec:system}

We take a data-driven approach to learn the cost function. Learning the cost
have many advantages over hand-designed heuristics and it has been shown to help
in
many applications (e.g.,~\cite{Abbeel10,Kober11,Ratliff06}). Furthermore, a
learned
cost function  can adapt as more data becomes available while the heuristics
remains fixed.
Particularly in our setting, an environment can be arbitrarily
complex (Fig.~\ref{fig:activities}) with many humans, objects, and
interactions between them. Heuristics do not
generalize well across such environments. In Section~\ref{subsec:discriminative} we
compare against few such heuristics.

\begin{figure*}[tb!]
\centering
\includegraphics[width=.8\linewidth]{system_picture3.jpg}
\caption{\textbf{An illustration of our PlanIt system.} Our learning system has
three main components (i) affordance
representation and cost parameterization; (ii) The PlanIt engine for receiving user
preference feedback; and (iii) Learning algorithm.}
\label{fig:system}
\end{figure*}

User preference data on robot trajectories is challenging to obtain and is not
readily available.
We build a learning system which makes it easy for users to
reveal their preferences and allows the learned model to improve as more data
becomes available. Our system is closed loop, Fig.~\ref{fig:system}, wherein the robot
learns from user feedback.

We maintain an affordance library of spatial distributions for each human
activity. When a robot observes an environment, it uses distributions from the
library and builds a planning affordance map (Section~\ref{sec:representation}).
It then samples trajectories using
the cost function and presents them on the PlanIt engine for
user feedback (Section~\ref{subsec:planit}). After observing the feedback, the
model parameters are updated for
future environments (Section~\ref{subsec:learning}).
% \footnote{In our current experiments we update parameters in
% a batch manner i.e. after certain feedback iterations.}
In the following
sections, we explain each of the components of our system.

